No-regret Learning in Price Competitions under Consumer Reference Effects

We study long-run market stability for repeated price competitions between two firms, where consumer demand depends on firms' posted prices and consumers' price expectations called reference prices. Consumers' reference prices vary over time according to a memory-based dynamic, which is a weighted average of all historical prices. We focus on the setting where firms are not aware of demand functions and how reference prices are formed but have access to an oracle that provides a measure of consumers' responsiveness to the current posted prices. We show that if the firms run no-regret algorithms, in particular, online mirror descent(OMD), with decreasing step sizes, the market stabilizes in the sense that firms' prices and reference prices converge to a stable Nash Equilibrium (SNE). Interestingly, we also show that there exist constant step sizesunder which the market stabilizes. We further characterize the rate of convergence to the SNE for both decreasing and constant OMD step sizes.

==> 06_broaderimpact.tex <==
\newpage
\section*{Broader Impact}
\vspace{-0.3cm}
%This work sheds light on market stability concerning competition among multiple firms under consumer reference effects. As discussed at the very beginning of the introduction, market stability is an important feature for business organizations and entities who are interacting in complex and highly dynamic environments, as it presents firms with favorable market conditions under which they can better understand market behavior to guide long-term decision making. 
This work sheds light on market stability concerning competition among multiple firms under consumers' reference effects. As discussed at the very beginning of the introduction, market stability is an important feature for business organizations and entities who are interacting in complex and highly dynamic environments. In a stable market, firms can better understand market behavior to guide their long-term decision making. This work shows that firms can obtain the desired market stability condition by running simple off-the-shelf online algorithms such as OMD. These algorithms do not require a large amount of information about market characteristics and perform very well in a dynamic competitive environments. 


In many e-commerce and online retail platforms, automated learning and pricing algorithms are prevalent. Thus, 
we believe that our paper provides firms with a simple automated solution for complex dynamic pricing decisions,  which may potentially lead to stable markets.
% \negin{I was a huge fan of this part, ``Although this work does not intend to present firms with guidance on how to achieve market stability as a whole, we believe that our analysis of stability properties under opaque environments may potentially provide important implications for decision makers  to better understand the patterns of competitive activity under consumer reference effects. In turn, such understanding may prevent firms from overreacting to specific market phenomena or take radical actions, which can both have disruptive effects to market conditions and hence endanger consumer welfare." Let's discuss it.}
%Although this work does not intend to present firms with guidance on how to achieve market stability as a whole, we believe that our analysis of stability properties under opaque environments may potentially provide important implication for firm decision makers  to better understand the patterns of competitive activity under consumer reference effects. In turn, such understanding may prevent firms from overreacting to specific market phenomena or take radical actions, which can both have disruptive effects to market conditions and hence endanger consumer welfare.

\begin{ack}
This work was partially supported by the Office of Naval Research (ONR) grant N00014-18-1-2122.
\end{ack}

==> 06_technical.tex <==
\section{Proofs for Key Theorems}
\label{sec:technical}
In this section, we will provide proofs for some of our main results.

\begin{definition}[Best response mapping] 
We define the best-response mapping as $\bm{\psi}:\mathcal{P}^{3} \to \mathcal{P}^{2}$ such that $\bm{\psi}(\bm{p},r) = \left(\psi_{1}(p_{2},r), \psi_{2}(p_{1},r) \right)$. Then, we can rewrite the set of best-response profiles w.r.t. reference price $r$, defined in Equation (\ref{eq:NE:bestresponseprfile}), as $\mathcal{B}(r) = \left\{\bm{p} \in \mathcal{P}^{2}: \bm{p} = \bm{\psi}(\bm{p},r)\right\}$. Note that for any SNE $(\bm{p}^{*},r^{*})$, we must have $\bm{p}^{*}\in \mathcal{B}(r^{*})$, and $\bm{p}^{*}$ is a fixed point of the mapping $\bm{\psi}(\cdot,r^{*})$.
\end{definition}
\begin{definition}[Bregman Divergence]
\label{def:BD}
The Bregman divergence $ \BD: \mathcal{C} \times \mathcal{C} \to \R^+$ associated with convex set $\mathcal{C}\subset \R$, and convex and continuously differentiable function $R: \mathcal{C} \to \R$ is defined as $ \BD(x,y) \defeq R(x) - R(y) - R'(y) (x-y) \geq 0$, where the inequality follows from convexity of $R$. Furthermore, if $R$ is $\sigma$-strongly convex, then $ \BD(x,y) \geq \frac{\sigma^2}{2}(x-y)^{2}$.
\end{definition}
We denote $\BDi$ as the Bregman divergence associated with regularizer $R_i$ used by firm $i=1,2$, and $\BDn$ as the Bregman divergence associated with regularizer $R_n$ used by nature.
\begin{definition}
Let $g_i^{*}$ be the partial derivative of the cost function $\widetilde{\pi}_{i}$ w.r.t. $p_{i}$ evaluated at the interior SNE $(\bm{p}^{*},r^{*})$, i.e. for $i=1,2,n$, $g_i^* = \frac{\partial \widetilde{\pi}_{i}(p_{1},p_{2},p_{n})}{\partial p_i}\Big|_{p_{1} = p_{1}^{*}, p_{2} = p_{2}^{*}, p_{n} = r^{*}}$.
\end{definition}


\subsection{Proof of Theorem \ref{thm:NEconvergence}}
\label{sec:technical:3.1}
(i) By first order conditions, we know that $\arg\max_{p\in \R} \pi_{i}(p,p_{-i},r) =\frac{\alpha_{i} + \delta_{i} p_{-i} + \gamma_{i} r }{2\beta_{i}}$. Hence, due to boundary constraints on the decision set $\mathcal{P}$ and the revenue function being quadratic, we have \[\psi_{i}(p_{-i},r) =\arg\max_{p\in \mathcal{P}} \pi_{i}(p,p_{-i},r)= \Pi_{\mathcal{P}}\left(\frac{\alpha_{i} + \delta_{i} p_{-i} + \gamma_{i} r }{2\beta_{i}}\right)\,,\] where $\Pi_{\mathcal{P}}:\R \to \mathcal{P}$ is the projection operator such that $\Pi_{\mathcal{P}}(z) = z \I\{z \in \mathcal{P}\} + \underline{p} \I\{z < \underline{p}\}+\Bar{p} \I\{z > \Bar{p}\}$. Hence, $\psi_{i}(p_{-i},r)$ is a nondecreasing function in $p_{-i}$ and $r$, which further implies $\bm{\psi}(\bm{p},r)$ is nondecreasing in $\bm{p}$ and $r$. Again, recall for any $\bm{x}, \bm{y}$, the relationships $\bm{x} \leq \bm{y}$ and $\bm{y} \leq \bm{x}$ are component-wise comparisons. 


We now follow a similar proof to that of Tarski's fixed point theorem: consider the set $\mathcal{B}_{+}(r) = \left\{\bm{p} \in \mathcal{P}^{2}: \bm{p}\leq \bm{\psi}(\bm{p},r) \right\}$. It is apparent that this set is nonempty because $(\underline{p},\underline{p}) \in \mathcal{B}_{+}(r)$. Fix any $\bm{p} \in \mathcal{B}_{+}(r)$. Then, we have $\bm{p}\leq \bm{\psi}(\bm{p},r)$ which further implies $\bm{\psi}(\bm{p},r)\leq \bm{\psi}\left(\bm{\psi}(\bm{p},r), r\right)$ since 
$\bm{\psi}(\bm{p},r)$ is nondecreasing in $\bm{p}$. Hence $\bm{\psi}(\bm{p},r) \in \mathcal{B}_{+}(r)$. By taking $\bm{U}(r) = \sup \mathcal{B}_{+}(r)$ (this is possible since all $\bm{p} \in \mathcal{B}_{+}(r)$ are bounded), we have $\bm{p} \leq \bm{U}(r)$ so  $\bm{p} \leq \bm{\psi}(\bm{p},r)\leq \bm{\psi}(\bm{U}(r),r)$. This further implies $\bm{U}(r)\leq \bm{\psi}(\bm{U}(r),r)$ because $\bm{U}(r)$ is the least upper bound of $\mathcal{B}_{+}(r)$, and thus $\bm{U}(r) \in\mathcal{B}_{+}(r) $. This allows us to conclude $ \bm{\psi}(\bm{U}(r),r) \leq \bm{U}(r)$ and hence $\bm{U}(r) = \bm{\psi}(\bm{U}(r),r)$, which means $\bm{U}(r) = \sup \mathcal{B}_{+}(r)$ is a fixed point of the mapping $\bm{\psi}(\cdot, r)$. Thus,  $\bm{U}(r)$ belongs in the set of best-response profiles $\mathcal{B}(r)$, confirming $\mathcal{B}(r)$ is not empty. 

% q_{i} \I\left\{  q_{i} \in \mathcal{P} \right\} + \underline{p} \I\left\{  q_{i}< \underline{p} \right\} + \Bar{p} \I\left\{  q_{i} > \Bar{p} \right\} $
% where $q_{i} = \frac{\alpha_{i} + \delta_{i} p_{-i} + \gamma_{i} r }{2\beta_{i}}$

Next, we  show that $ \mathcal{B}(r)$ is an ordered set with total ordering if it is not a singleton. To do so,  consider any $\bm{p}, \bm{q} \in \mathcal{B}(r)$ and without loss of generality assume $p_{1} > q_{1}$. Since $p_{1}  = \psi_{1}(p_{2},r)$ and $q_{1} =\psi_{1}(q_{2},r) $, by monotonicity of $\psi_{1}(\cdot,r)$ we have $p_{2} > q_{2}$. Thus, $\bm{p} >  \bm{q}$ and $ \mathcal{B}(r)$ is an ordered set with total ordering. 

(ii) In the proof of (i), we showed that $\bm{U}(r)= \sup \left\{\bm{p} \in \mathcal{P}^{2}: \bm{p}\leq \bm{\psi}(\bm{p},r) \right\}$ is a fixed point of the best-response mapping $\bm{\psi}(\cdot,r)$ for any $r$
which allows us to conclude $\bm{U}(r)$ is the largest best-response profile, i.e., $\bm{U}(r) = \max \mathcal{B}(r)$, and hence $\bm{p}_{t} = \bm{U}(r_{t})$. Furthermore, since $\bm{\psi}(\bm{p},r)$ is increasing in $r$, we know that $\bm{U}(\cdot)= \sup \left\{\bm{p} \in \mathcal{P}^{2}: \bm{p}\leq \bm{\psi}(\bm{p},\cdot) \right\}$ is also an increasing function. In the following, we will argue that the reference prices $r_{t}$ is monotonically increasing or decreasing, which implies  $\bm{p}_{t} = \bm{U}(r_{t})$ is also monotonic, and hence converges since prices and reference prices are bounded.

We write $\bm{U}(r) = \left(U_{1}(r), U_{2}(r)\right)$. At $t=1$, if $\theta_1 p_{1,1}  + \theta_2 p_{2,1} = \theta_1 U_{1}(r_{1})  + \theta_2 U_{2}(r_{1}) \geq r_{1}$, then the reference price at $t=2$ satisfies  $r_{2} = ar_{1} + (1-a)\left( \theta_1 p_{1,1}  + \theta_2 p_{2,1}\right) \geq r_{1}$. By the  monotonicity of $\bm{U}(\cdot)$, we have $p_{i,2} = U_{i}(r_{2}) \geq U_{i}(r_{1}) = p_{i,1}$ for $i = 1,2$. Thus,  
\begin{align*}
    r_{3} ~=~ ar_{2} + (1-a)\left( \theta_1 p_{1,2}  + \theta_2 p_{2,2}\right) 
~\geq~  ar_{1} + (1-a)\left( \theta_1 p_{1,1}  + \theta_2 p_{2,1}\right) 
~=~ r_{2}\,.
\end{align*}
A simple induction argument thus shows $\{r_{t}\}_t$ is a nondecreasing sequence. Since $r_{t} \leq \Bar{p}$ for any $t \in \N$, we know that $\{r_{t}\}_t$ converges to some number $r_{+} \in [\underline{p},\Bar{p}]$ when $\theta_1 p_{1,1}  + \theta_2 p_{2,1} \geq r_{1}$. Furthermore, we observe that $\lim_{t\to \infty}\bm{\psi}(\bm{U}(r_{t}), r_{t}) = \bm{\psi}(\bm{U}(r_{+}), r_{+})$  by the definition of $\bm{\psi}$. Also, from (i) we have $\bm{\psi}(\bm{U}(r_{t}), r_{t}) = \bm{U}(r_{t})$ and $\bm{\psi}(\bm{U}(r_{+}), r_{+}) = \bm{U}(r_{+})$ because $\bm{U}(r)$ is a fixed point of $\bm{\psi}(\cdot, r)$ for any $r$. Hence, $\lim_{t\to \infty}\bm{U}(r_{t}) =\bm{U}(r_{+}) $, which implies $\{\bm{p}_{t} = \bm{U}(r_{t})\}_t$ converges to $\bm{U}(r_{+})$. Note that convergence is monotonic because $\bm{U}(\cdot)$ is nondecreasing. Therefore, 
$$\theta_{1}U_{1}(r_{+}) + \theta_{2}U_{2}(r_{+}) = \lim_{t\to\infty} \theta_{1}U_{1}(r_{t}) + \theta_{2}U_{2}(r_{t}) =  \lim_{t\to\infty} r_{t+1} =  r_{+}\,,$$
which implies $\left(\bm{U}(r_{+}), r_{+} \right)$ is an SNE. We can thus conclude that if $\theta_1 p_{1,1}  + \theta_2 p_{2,1} = \theta_1 U_{1}(r_{1})  + \theta_2 U_{2}(r_{1}) \geq r_{1}$,
firms' prices and reference prices converge monotonically to an SNE $\left(\bm{U}(r_{+}), r_{+} \right)$.

Following a symmetric argument, if $\theta_1 p_{1,1}  + \theta_2 p_{2,1} < r_{1}$, we can show that 
$\{r_{t}\}_t$ is a nonincreasing sequence.  Since  
$r_{t} \geq \underline{p}$ for any $t \in \N$, we know that $\{r_{t}\}_t$ converges to some number $r_{-} \in [ \underline{p},\Bar{p}]$. Similar to the previous arguments, we can conclude  that prices and reference prices converge monotonically to an SNE $\left(\bm{U}(r_{-}), r_{-} \right)$.
\Halmos



\subsection{Proof for Theorem \ref{thm:OMD:convergenceSufDecStep}}
\label{sec:technical:5.1}

The proof of this theorem is divided into two parts. In the first part, we show that the price profiles $\left(\bm{p}_{t}, r_{t}\right)$ converge  as $t \to \infty$ under the condition $\lim_{t \to \infty} \epsilon_{i,t} =  0$, $i\in \{1,2\}$. In the second part, under the additional conditions $\lim_{T \to \infty}\sum_{t=1}^{T}\epsilon_{i,t} = \infty$ and $\lim_{T \to \infty}\sum_{t=1}^{T}\epsilon_{i,t}^{2} < \infty $, we show that the price profiles converge to the unique interior SNE.


\textbf{First part: Convergence of prices and reference prices.} Recall that  $g_{i,t} = g_{i}(p_{i,t},r_{t}) = 2\beta_i p_{i,t} - \left(\alpha_i + \delta_i p_{-i,t} + \gamma_i r_{t} \right)$,  and $p_{i,t}$ and $p_{-i,t}  $ are both bounded. Hence, because for $i = 1,2$,  $\lim_{t \to \infty} \epsilon_{i,t} =  0$ and $\{ \epsilon_{i,t}\}_{t}$ is nonincreasing, we have for any small $\epsilon > 0$ there exist $ \te \in \N$ such that $|\epsilon_{i,t} g_{i,t}|\leq \frac{\sigma_{i}^{2}\epsilon}{6}$ for all $t > \te$. Our goal is to show that for $t\ge \te$, $|p_{i, t+1} - p_{i,t}|$ is small, and hence $\bm{p}$ converges. 
For $t > \te$,
\begin{align}
\label{eq:OMD:convergenceSufDecStep1}
    \left| p_{i,t+1} -p_{i,t} \right| ~\leq~ &  \left| p_{i,t+1} -y_{i,t+1} \right| + \left| y_{i,t+1} -p_{i,t} \right|
    ~\overset{(a)}{\leq}~  \left| p_{i,t+1} -y_{i,t+1} \right| + \frac{\epsilon}{6}\,. %\\
    % ~=~ &  \left| p_{i,t+1} -y_{i,t+1} \right|\left(\I\{y_{i,t+1} < \underline{p}\}+ \I\{y_{i,t+1}\in \mathcal{P}\} + \I\{y_{i,t+1} > \Bar{p}\} \right) + \frac{\epsilon}{12} \nonumber \\
    %  ~\overset{(b)}{=}~ &  \left| p_{i,t+1} -y_{i,t+1} \right|\left(\I\{y_{i,t+1} < \underline{p}\}+ \I\{y_{i,t+1} > \Bar{p}\} \right) + \frac{\epsilon}{12} 
\end{align}
To see why inequality (a) holds recall that  $y_{i,t+1}$ is the proxy variable in Step 5 of Algorithm \ref{algo:firmOMD} such that
% recall that  $y_{i,t+1}$ is the proxy variable in Step 5 of Algorithm \ref{algo:firmOMD} such that \negin{$\frac{dR_{i}(y_{i,t+1})}{dy}$ is confusing as it is not obvious why $y$ is. Can you use prime $'$ instead to show derivative? } 
$R_{i}'(y_{i,t+1}) - R_{i}'(p_{i,t}) = \epsilon_{i,t} g_{i,t}$. Hence,
% $\frac{dR_{i}(y_{i,t+1})}{dy}- \frac{dR_{i}(p_{i,t})}{dy}= \epsilon_{i,t} g_{i,t} $, we have 
\begin{align*}
    \sigma_{i}^{2}\left|y_{i,t+1} -  p_{i,t}\right|{\leq}\left|R_{i}'(y_{i,t+1}) - R_{i}'(p_{i,t}) \right| =  \left|\epsilon_{i,t} g_{i,t}\right| \leq \frac{\sigma_{i}^{2}\epsilon}{6}, \quad t> \te, i = 1,2\,,
\end{align*}
which implies that $\left| y_{i,t+1} -p_{i,t} \right|\le \frac{\epsilon}{6}$, as desired. 
Here,  the first inequality holds because:
\begin{align*}  
\sigma_{i}^{2}\left( y_{i,t+1} -  p_{i,t}\right)^{2}& ~\overset{(a)}{\leq}~ \left(R_{i}'(y_{i,t+1}) - R_{i}'(p_{i,t})\right)\left( y_{i,t+1} -  p_{i,t}\right) ~\leq~ \left|R_{i}'(y_{i,t+1}) - R_{i}'(p_{i,t})\right| \cdot \left|y_{i,t+1} -  p_{i,t} \right|\,,
\end{align*}
where (a) follows from summing up $R_{i}(y_{i,t+1}) - R_{i}(p_{i,t}) \geq R_{i}'(p_{i,t})(y_{i,t+1} - p_{i,t}) + \frac{\sigma_{i}^{2}}{2}\left( y_{i,t+1} -  p_{i,t}\right)^{2}$ and $R_{i}(p_{i,t}) - R_{i}(y_{i,t+1}) \geq R_{i}'(y_{i,t+1})(p_{i,t} - y_{i,t+1}) + \frac{\sigma_{i}^{2}}{2}\left( y_{i,t+1} -  p_{i,t}\right)^{2} $ due to strong convexity. 


By Equation \eqref{eq:OMD:convergenceSufDecStep1}, for $t > \te$,
\begin{align}
    \left| p_{i,t+1} -p_{i,t} \right| 
     ~\le~ &  \left| p_{i,t+1} -y_{i,t+1} \right|\left(\I\{y_{i,t+1} < \underline{p}\}+ \I\{y_{i,t+1}\in \mathcal{P}\} + \I\{y_{i,t+1} > \Bar{p}\} \right) + \frac{\epsilon}{6} \nonumber \\
      ~{=}~ &  \left| p_{i,t+1} -y_{i,t+1} \right|\left(\I\{y_{i,t+1} < \underline{p}\}+ \I\{y_{i,t+1} > \Bar{p}\} \right) + \frac{\epsilon}{6}\,,
\end{align}
where the equality holds because under the event $y_{i,t+1}\in \mathcal{P}$, no projection occurs and hence, $y_{i,t+1} = p_{i,t+1}$. In the first of the proof, we bound the first two terms in the right hand side, i.e., $\left| p_{i,t+1} -y_{i,t+1} \right|\I\{y_{i,t+1} < \underline{p}\}$ and  $\left| p_{i,t+1} -y_{i,t+1} \right|\I\{y_{i,t+1} > \Bar{p}\}$. 


To bound $\left| p_{i,t+1} -y_{i,t+1} \right|\I\{y_{i,t+1} < \underline{p}\}$, similar to Equation (\ref{eq:OMD:convergenceSufDecStep1}) we use $|p_{i,t}  - y_{i,t+1}| \leq \frac{\epsilon}{6}$ for $t > \te$ which implies $p_{i,t}  - y_{i,t+1} \leq \frac{\epsilon}{6}$. Thus,
\begin{align}
\label{eq:OMD:convergenceSufDecStep1.1}
 y_{i,t+1} \geq p_{i,t} - \frac{\epsilon}{6} \overset{(a)}{\geq} \underline{p} - \frac{\epsilon}{6}\,.
\end{align}
where (a) holds because $p_{i,t}  \geq \underline{p}$ for any $i,t$. On the other hand,  under the event $y_{i,t+1} < \underline{p}$, projection occurs and therefore we have $p_{i,t+1} = \underline{p}$. 
% To see why,  recall $p_{i,t} = \arg\min_{p\in \mathcal{P}} \BDi(p, y_{i,t})$. It is easy to verify that $\frac{d\BDi(p, y_{i,t})}{dp} = \frac{dR_i(p)}{dp} - \frac{dR_i(p)}{dp}\Big|_{p = y_{i,t}}$. Convexity of $R_i$ implies that $\frac{dR_i(p)}{dp}$ is nondecreasing in $p$, so $\frac{d\BDi(p, y_{i,t})}{dp} = \frac{dR_i(p)}{dp} - \frac{dR_i(p)}{dp}\Big|_{p = y_{i,t}}\geq 0$  for all $p \geq y_{i,t}$. This shows $\BDi(p, y_{i,t}) $ is nondecreasing on $[y_{i,t},\infty)$ and hence nondecreasing on $\mathcal{P} = [\underline{p},\Bar{p}]$ given  $y_{i,t} < \underline{p}$. Thus $\BDi(\underline{p}, y_{i,t}) \leq \BDi(p, y_{i,t})$ for any $p \in \mathcal{P}$, so $p_{i,t} = \arg\min_{p\in \mathcal{P}} \BDi(p, y_{i,t}) = \underline{p}$. \negin{By going with a simpler projection step, you can remove the above argument.} 
This yields
\begin{align}
    \left| p_{i,t+1} -y_{i,t+1} \right|\I\{y_{i,t+1} < \underline{p}\} = \left( \underline{p} - y_{i,t+1}\right)\I\{y_{i,t+1} < \underline{p}\} \overset{(a)}{\leq}\left( \underline{p} - \underline{p} + \frac{\epsilon}{6}\right) =  \frac{\epsilon}{6}\,,
\end{align}
where (a) follows from Equation (\ref{eq:OMD:convergenceSufDecStep1.1}).

Using a similar argument as above to bound $\left| p_{i,t+1} -y_{i,t+1} \right|\I\{y_{i,t+1}> \high\}$, we have $ \left| p_{i,t+1} -y_{i,t+1} \right|\I\{y_{i,t+1} >  \Bar{p}\}\leq \frac{\epsilon}{6}$ under the event $y_{i,t+1} > \Bar{p}$. Plugging these upper bounds back into Equation (\ref{eq:OMD:convergenceSufDecStep1}), we can show that  for any $\epsilon > 0$ and $ t > \te$
\begin{align}
\label{eq:OMD:convergenceSufDecStep2}
    \left| p_{i,t+1} -p_{i,t} \right| ~\leq~ \frac{\epsilon}{6} + \frac{\epsilon}{6}+\frac{\epsilon}{6}~=~ \frac{\epsilon}{2}, \quad  i = 1,2 \,.
\end{align}
This shows prices converge, i.e., $\bm{p}_{t}$ converges.

Finally, we use the convergence of $\bm{p}_{t}$ to show that reference prices also converge. When  $t> \te$,
\begin{align*}
    \left| r_{t+2} - r_{t+1}\right| ~\leq~ & a\left|r_{t+1} - r_{t} \right|  + (1-a)\sum_{i=1,2}\theta_{i}\left|p_{i,t+1} -p_{i,t} \right|
    ~\overset{(a)}{\leq}~ a\left|r_{t+1} - r_{t} \right|  + \frac{(1-a)\epsilon}{2}\,,
\end{align*}
where (a) follows from the convergence of $p_{i,t}$ in Equation (\ref{eq:OMD:convergenceSufDecStep2}). Rearranging terms, this yields $ \left| r_{t+2} - r_{t+1}\right|  - \frac{\epsilon}{2}~\leq~ a\left(\left|r_{t+1} - r_{t} \right|  - \frac{\epsilon}{2}\right)$. Using a telescoping argument, we have 
\begin{align*}
    \left| r_{t+2} - r_{t+1}\right|  - \frac{\epsilon}{2}~\leq~ a^{t}\left(\left|r_{2} - r_{1} \right|  - \frac{\epsilon}{2}\right)\leq a^{t}\left(\Bar{p}  -\underline{p} - \frac{\epsilon}{2}\right) \,.
\end{align*}
Since $a \in (0,1)$, there exists  $\exists \ta \in \N$ such that  $\left| r_{t+2} - r_{t+1}\right|  - \frac{\epsilon}{2} \leq \frac{\epsilon}{2}$ for all $t > \ta$. Therefore, for any $t > \max \{ \te,\ta\}$, $ \left| p_{i,t+1} -p_{i,t} \right| \leq \frac{\epsilon}{2}$ and $ \left| r_{t+2} - r_{t+1}\right| \leq \epsilon$. This implies  $\left(\bm{p}_{t}, r_{t}\right)$ converges as $t \to \infty$.




\textbf{Second part: Convergence to the SNE.} Now we show, via a contradiction argument,  that if the conditions $\lim_{T \to \infty}\sum_{t=1}^{T}\epsilon_{i,t} = \infty$ and $\lim_{T \to \infty}\sum_{t=1}^{T}\epsilon_{i,t}^{2} < \infty$ hold, then $\left(\bm{p}_{t}, r_{t}\right)$ converges to the interior SNE $\left(\bm{p}^{*}, r^{*}\right)$. Here, we first provide a roadmap of the proof:

{We start by evoking Corollary \ref{cor:SNEBregmanUpdate}: for any $i=1,2,n$ and $t\in \N^{+}$, we get
\begin{align}
\label{eq:OMD:standardAnalysis1}
 \BDi(p_i^*, p_{i,t+1})
     ~\leq~  \BDi(p_i^*, p_{i,t})  - \epsilon_{i,t}\left(g_i^{*} - g_{i,t}\right)\left( p_i^{*} - p_{i,t} \right) +  \frac{\left(\epsilon_{i,t}\right)^2 g_{i,t}^{2}}{2\sigma_i} \,,
\end{align}
where we recall $g_i^{*}$ is the partial derivative of the cost function $\widetilde{\pi}_{i}$ w.r.t. $p_{i}$ evaluated at the interior SNE $(\bm{p}^{*},r^{*})$. If contrary to our claim,  prices for firm $i$  converge to some point other than the SNE prices, we can lower bound $\left(g_i^{*} - g_{i,t}\right)\left( p_i^{*} - p_{i,t} \right)$ with some positive constant. Then, by utilizing the aforementioned step size conditions, we show that, roughly speaking, the distance between $p_{i,t}$ and $p_{i}^{*}$, measured by $\BDi(p_i^*, p_{i,t})$, decreases by a constant amount for each time period after large enough $t$. Eventually, this tells us that the distance between  $p_{i,t}$ and $p_{i}^{*}$ will become negative, leading to a contradiction regarding the Bregman Divergence being positive. We conduct our proof in 3 steps. {In Step 1, we provide bounds for $g_i^{*} - g_{i,t}$ (bounds for $p_i^{*} - p_{i,t}$ are relatively easy to show); in Step 2 we lower bound $\left(g_i^{*} - g_{i,t}\right)\left( p_i^{*} - p_{i,t} \right)$ for large enough $t$ if firm $i$'s prices converge to some point other than the  SNE; and in Step 3, we show that the positive lower bound for $\left(g_i^{*} - g_{i,t}\right)\left( p_i^{*} - p_{i,t} \right)$ will eventually lead to a contradiction regarding Bregman Divergence being positive.}}
% in Step 1, we show that assuming we can lower bound $\left(g_i^{*} - g_{i,t}\right)\left( p_i^{*} - p_{i,t} \right)$ with a positive number, we arrive at a contradiction (w.r.t Bregman Divergence being positive); In Step 2, we provide bounds for $g_i^{*} - g_{i,t}$ (bounds for $p_i^{*} - p_{i,t}$ are relatively easy to show); In Step 3, we lower bound $\left(g_i^{*} - g_{i,t}\right)\left( p_i^{*} - p_{i,t} \right)$ if firm $i$'s prices converge to some point other than the  SNE, and then evoke Step 1 to show a contradiction. }


 To begin with, contrary to our claim, assume that  $\left(\bm{p}_{t}, r_{t}\right) \overset{t \to \infty}{\longrightarrow} \left(\widetilde{\bm{p}}, \widetilde{r}\right) \neq \left(\bm{p}^{*}, r^{*}\right)$, and define $\Delta_i = p_i^{*} - \widetilde{p}_{i}$ for $i = 1,2,n$. Fix $\ell \in \{1,2\}$ such that %\negin{Why are you changing $i$  to $\ell$?}\jasoncom{$i$ is a general firm, where $\ell$ is a specific firm, so using $i$ will be very confusing. I tried using $\widetilde{i}$ but it is very messy. We can also use $j$ if you want...}
 $|\Delta_{\ell}| \geq |\Delta_{-\ell}| \geq 0$ that is, let $\ell$ be the firm whose corresponding $|\Delta_{\ell}|$ is most far away from 0. Since $\left(\widetilde{\bm{p}}, \widetilde{r}\right) \neq \left(\bm{p}^{*}, r^{*}\right)$, we know that $|\Delta_{\ell}| > 0$ and hence $\Delta_{\ell} \neq 0$. Note that it is possible that the other firm $-\ell$ has $\Delta_{-\ell} = 0$. Define $\eta$ such that 
 \begin{align}
\label{eq:OMD:NEDeviationEq}
    0 < \eta ~<~ \min\left\{\frac{\left| \left(2\beta_{\ell} - \gamma_{\ell}\theta_{\ell}\right)\Delta_{\ell} - \left( \gamma_{\ell}\theta_{-\ell} + \delta_{\ell}  \right)\Delta_{-\ell} \right|}{2\beta_{\ell} + \delta_{\ell} + \gamma_{\ell}} ,\frac{ 2\beta_{\ell} - \gamma_{\ell}\theta_{\ell}}{2\beta_{\ell} + \delta_{\ell} + \gamma_{\ell}}\left|\Delta_{\ell}\right|\right\}\,.
\end{align}
First, note that such an $\eta$ exists because $\left|\Delta_{\ell}\right| > 0$ and $\left| \left(2\beta_{\ell} - \gamma_{\ell}\theta_{\ell}\right)\Delta_{\ell} - \left( \gamma_{\ell}\theta_{-\ell} + \delta_{\ell}  \right)\Delta_{-\ell} \right| \overset{(a)}{>} 0$. Here, (a) is due to the fact that $\beta_{\ell}\ge \margin(\delta_{\ell}+\gamma_{\ell})$ with $\margin\ge 2$, and $\theta_{\ell}\in (0,1)$, which implies
$ 2\beta_{\ell} - \gamma_{\ell}\theta_{\ell} > \gamma_{\ell}\theta_{-\ell} + \delta_{\ell}  > 0$, and 
$$\left| \left(2\beta_{\ell} - \gamma_{\ell}\theta_{\ell}\right)\Delta_{\ell} - \left( \gamma_{\ell}\theta_{-\ell} + \delta_{\ell}  \right)\Delta_{-\ell} \right| > \left( 2\beta_{\ell} - \gamma_{\ell}\theta_{\ell}\right) \cdot \left|\Delta_{\ell}\right| - \left( \gamma_{\ell}\theta_{-\ell} + \delta_{\ell}  \right) \cdot \left|\Delta_{-\ell} \right| \overset{(b)}{>} 0,$$
where in (b) we also used the fact that $|\Delta_{\ell}| \geq |\Delta_{-\ell}| \geq 0$ and  $|\Delta_{\ell}| > 0$.
Also, note that definition of $\eta$  implies that we have $0 < \eta < \left|\Delta_{\ell}\right|$ as for any $i = 1,2$, $0 < \frac{2\beta_{i} - \gamma_{i}\theta_{i}}{2\beta_{i} + \delta_{i} + \gamma_{i}} <1$. 

Furthermore, because$\left(\bm{p}_{t}, r_{t}\right) $ converges to $\left(\widetilde{\bm{p}}, \widetilde{r}\right)$, let $\teta \in \N^{+}$ be the period such that $\left|\widetilde{p}_{i} - p_{i,t}\right| < \eta$ for all $t > \teta$ and $i = 1,2,n$. This allows us to characterize the distance between prices and the SNE for $i=1,2$ and $t > \teta$: 
\begin{align}
 &  p_{{i}}^{*} - p_{{i},t} = p_{{i}}^{*} - \widetilde{p}_{{i}} +  \widetilde{p}_{{i}} - p_{{i},t} <  \Delta_{{i}} + \eta \label{eq:OMD:priceUB}\\
     & p_{{i}}^{*} - p_{{i},t} = p_{{i}}^{*} - \widetilde{p}_{{i}} - \widetilde{p}_{{i}} - p_{{i},t} >  \Delta_{{i}} - \eta \label{eq:OMD:priceLB}\,.
\end{align}


\textbf{Step 1.} 
 Here, we will show the following lower and upper bounds for $g_{\ell}^{*} - g_{\ell,t}$ for any $t > \teta$: 
\begin{align}
  &  g_{\ell}^*- g_{\ell,t} 
  ~\leq~  \left(2\beta_{\ell}  - \gamma_{\ell} \theta_{\ell} \right)\Delta_{\ell} - \left(\delta_{\ell} + \gamma_{\ell} \theta_{-\ell} \right)\Delta_{-\ell} + \eta\left(2\beta_{\ell}  + \delta_{\ell} +\gamma_{\ell} \right)  \label{eq:OMD:grad1diffUB}\\
  &  g_{\ell}^*- g_{\ell,t} 
  ~\geq~ \left(2\beta_{\ell}  - \gamma_{\ell} \theta_{\ell} \right)\Delta_{\ell} - \left(\delta_{i} + \gamma_{\ell} \theta_{-\ell} \right)\Delta_{-\ell} - \eta\left(2\beta_{\ell}  + \delta_{\ell} +\gamma_{\ell} \right) \label{eq:OMD:grad1diffLB} \,.
\end{align}
\begin{itemize}[leftmargin=*]
    \item \textbf{Lower bounding $\bf{g_{\ell}^*- g_{\ell,t}}$.} Recall $g_{\ell}(p_{\ell},p_{-\ell},r) = 2\beta_{\ell}p_{\ell} - \left(\alpha_{\ell} + \delta_{\ell} p_{-\ell} + \gamma_{\ell} r  \right)$, $g_{\ell,t} = g_{\ell}(\bm{p}_{t},r_{t})$ and $g_{\ell}^{*} = g_{\ell}(\bm{p}^{*},r^{*})$. Then,
    \begin{align}
    \label{eq:OMD:gradDiffEq}
    g_{\ell}^*- g_{\ell,t} 
    ~=~ &2\beta_{\ell} \left( p_{\ell}^{*} - p_{\ell,t}\right)-  \delta_{\ell}\left(p_{-\ell}^{*} -  p_{-\ell,t}\right) - \gamma_{\ell} \left(r^{*} - r_{t} \right) \,.
\end{align}
Therefore, for $t > \teta$ we have
\begin{align*}
  g_{\ell}^*- g_{\ell,t} 
  ~=~ & 2\beta_{\ell} \left( p_{\ell}^{*} - \widetilde{p}_{\ell} +  \widetilde{p}_{\ell} - p_{\ell,t}\right) -  \delta_{\ell}\left(p_{-\ell}^{*} - \widetilde{p}_{-\ell} +  \widetilde{p}_{-\ell} -  p_{-\ell,t}\right) - \gamma_{\ell} \left(r^{*} - \widetilde{r} + \widetilde{r} - r_{t} \right) 
  \nonumber  \\
  ~\overset{(a)}{\geq}~ & 2\beta_{\ell} \left(\Delta_{\ell} - \eta \right)-  \delta_{\ell}\left(\Delta_{-\ell} + \eta \right) - \gamma_{\ell} \left(\Delta_{n} + \eta \right)\nonumber  \\
  ~\overset{(b)}{=}~ & \left(2\beta_{\ell}  - \gamma_{\ell} \theta_{\ell} \right)\Delta_{\ell} - \left(\delta_{\ell} + \gamma_{\ell} \theta_{-\ell} \right)\Delta_{-\ell} - \eta\left(2\beta_{\ell}  + \delta_{\ell} +\gamma_{\ell} \right) \,,
\end{align*}
where (a) follows from the fact that  $|\widetilde{p}_{i} - p_{i,t}| \leq \eta$ for any $t > \teta$ and $i=1,2$, and (b) follows from the relationship $ \Delta_{n} = \theta_{1}\Delta_{1}
 + \theta_{2}\Delta_{2}$, which holds due to the following: 
 \begin{align*}
    \widetilde{r} = \lim_{t\to \infty} r_{t+1} = \lim_{t\to \infty} ar_{t} + (1-a)\left(\theta_{1}p_{1,t} + \theta_{2}p_{2,t}\right) = a\widetilde{r} + (1-a)\left(\theta_{1}\widetilde{p}_{1} + \theta_{2}\widetilde{p}_{2}\right)\,.
\end{align*}Combining this with  $r^{*} =\left(\theta_{1}p_{1}^{*} + \theta_{2}p_{2}^{*}\right)$ (due to the definition of the SNE), and the definition of $\Delta_{i} = p_{i}^{*} - \widetilde{p}_{i}$ for $i = 1,2,n$ yields the desired lower bound.
\item \textbf{Upper bounding $\bf{g_{\ell}^*- g_{\ell,t}}$.} Similar to the lower above, for $t > \teta$ we have
\begin{align*}
 g_{\ell}^*- g_{\ell,t} ~\leq~ & 2\beta_{\ell} \left(\Delta_{\ell}  + \eta \right)-  \delta_{\ell}\left(\Delta_{-\ell} - \eta \right) - \gamma_{\ell} \left(\Delta_{n}  - \eta \right)\nonumber  \\
  ~=~ & \left(2\beta_{\ell}  - \gamma_{\ell} \theta_{\ell} \right)\Delta_{\ell} - \left(\delta_{\ell} + \gamma_{\ell} \theta_{-\ell} \right)\Delta_{-\ell} + \eta\left(2\beta_{\ell}  + \delta_{\ell} +\gamma_{\ell} \right)\,.
\end{align*}
\end{itemize}


\textbf{Step 2.} 
If $\Delta_{\ell}  > 0$, then since $ 2\beta_{\ell} - \gamma_{\ell}\theta_{\ell} > \gamma_{\ell}\theta_{-\ell} + \delta_{\ell}  > 0$ and $|\Delta_{\ell}| \geq |\Delta_{-\ell}| \geq 0$, we have $ \left(2\beta_{\ell}  - \gamma_{\ell} \theta_{\ell} \right)\Delta_{\ell} - \left(\delta_{i} + \gamma_{\ell} \theta_{-\ell} \right)\Delta_{-\ell} > 0$. Using the lower bound in Equation (\ref{eq:OMD:grad1diffLB}),  we get for any $t > \teta$:
\begin{align*}
     g_{\ell}^*- g_{\ell,t} 
  ~\geq~ \left(2\beta_{\ell}  - \gamma_{\ell} \theta_{\ell} \right)\Delta_{\ell} - \left(\delta_{i} + \gamma_{\ell} \theta_{-\ell} \right)\Delta_{-\ell} - \eta\left(2\beta_{\ell}  + \delta_{\ell} +\gamma_{\ell} \right) \overset{(a)}{>} 0\,,
\end{align*}
where (a) follows from the definition of $\eta$ such that $\eta < \frac{ \left|\left(2\beta_{\ell} - \gamma_{\ell}\theta_{\ell}\right)\Delta_{\ell} - \left(\delta_{\ell} + \gamma_{\ell}\theta_{-\ell} \right)\Delta_{-\ell}\right|}{2\beta_{\ell} + \delta_{\ell} + \gamma_{\ell}}$. With $\Delta_{\ell}  > 0$, the lower bound in Equation (\ref{eq:OMD:priceLB}) implies  $p_{\ell}^{*} - p_{\ell,t} > \Delta_{\ell} - \eta > 0$ because $0 < \eta < |\Delta_{\ell}|$. Hence, by combining these lower bounds, we get for any $t > \teta$
\begin{align}
\label{eq:OMD:firstOrdergeq0}
    \left( p_{\ell}^{*} - p_{\ell,t} \right)  \left(g_{\ell}^{*} - g_{\ell,t}\right)
    >  |\Delta_{\ell} + \eta|\cdot \left|  \left(2\beta_{\ell}  - \gamma_{\ell} \theta_{\ell} \right)\Delta_{\ell} - \left(\delta_{\ell} + \gamma_{\ell} \theta_{-\ell} \right)\Delta_{-\ell} + \eta\left(2\beta_{\ell}  + \delta_{\ell} +\gamma_{\ell} \right)\right| \defeq \ceta > 0\,.
\end{align}
Similarly, if $\Delta_{\ell}  < 0$, then using the upper bounds in Equations (\ref{eq:OMD:grad1diffUB}) and (\ref{eq:OMD:priceUB}), we have $$ g_{\ell}^*- g_{\ell,t} 
  ~\leq~ \left(2\beta_{\ell}  - \gamma_{\ell} \theta_{\ell} \right)\Delta_{\ell} - \left(\delta_{i} + \gamma_{\ell} \theta_{-\ell} \right)\Delta_{-\ell} - \eta\left(2\beta_{\ell}  + \delta_{\ell} +\gamma_{\ell} \right) < 0$$ and $p_{\ell}^{*} - p_{\ell,t} < \Delta_{\ell} + \eta < 0$, which again allows us to obtain the lower bound  for $\left( p_{\ell}^{*} - p_{\ell,t} \right)  \left(g_{\ell}^{*} - g_{\ell,t}\right)$ in Equation (\ref{eq:OMD:firstOrdergeq0}).

\textbf{Step 3.} 
Telescoping Equation (\ref{eq:OMD:standardAnalysis1}) from $\teta+1$ to some large time period $T +1 > \teta + 1$, and applying the lower bound in Equation (\ref{eq:OMD:firstOrdergeq0}), i.e., $\left( p_{\ell}^{*} - p_{\ell,t} \right)  \left(g_{\ell}^{*} - g_{\ell,t}\right) \geq \ceta > 0$ for all $t > \teta$,  we get
\begin{align}
    \label{eq:OMD:telescope}
%   \frac{\sigma_{\ell}^2}{2}\left(|\Delta_{\ell}|- \eta \right)^2 
%   0~\overset{(a)}{\leq}
%   0~\leq~&  
   \BDl(p_{\ell}^*, p_{\ell,T+1}) 
    ~\leq~ \BDl(p_{\ell}^*, p_{\ell,T}) - \ceta \epsilon_{\ell,T} +  \V\epsilon_{\ell,T}^{2}
    % & \vdots \nonumber \\
   ~\overset{(a)}{\leq}~ \BDl(p_{\ell}^*, p_{\ell,\teta+1}) - \ceta\sum_{t= \teta+1}^{T} \epsilon_{\ell,t} +   \V\sum_{t= \teta+1}^{T} \epsilon_{\ell,t}^{2} \,,
\end{align}
where we take the absolute constant $\V > \max_{t \in \N} \frac{g_{\ell,t}^{2}}{2\sigma_{\ell}}$, which is possible as  the gradient $g_{\ell,t}$ is a linear function in all arguments and prices/reference prices are bounded, and in (a) we used a telescoping argument.
% Inequality (a) follows from strong convexity of $R_i$: $$\BDl(p_{\ell}^*, p_{\ell,T+1}) ~\geq~ \frac{\sigma_{\ell}^2}{2}\left(p_{\ell}^* - p_{\ell,T+1}\right)^{2} ~\overset{(b)}{\geq}~ 0 \,,$$ \frac{\sigma_{\ell}^{2}}{2}\left( \left| \Delta_{\ell}\right| - \eta\right)^{2}\,,
% where (b)
% follows from $|p_{\ell}^* - p_{\ell,t}| > |\Delta_{\ell} - \eta| \geq |\Delta_{\ell}| - \eta > 0$ for all $t > \teta$ by evoking the lower bound of $p_{\ell}^* - p_{\ell,t}$ in Equation (\ref{eq:OMD:priceLB}) and using the definition that $0 < \eta <  |\Delta_{\ell}|$. 
Since $\BDl(p_{\ell}^*, p_{\ell,T+1}) \geq 0$, rearranging terms in Equation \eqref{eq:OMD:telescope} and dividing both sides by $\sum_{t= \teta+1}^{T} \epsilon_{\ell,t}$ we get
the following:
\begin{align*}
   \frac{-\BDl(p_{\ell}^*, p_{\ell,\teta+1})}{\sum_{t= \teta+1}^{T} \epsilon_{\ell,t}}  ~\leq~   - \ceta +   \V \frac{\sum_{t= \teta+1}^{T} \epsilon_{\ell,t}^{2}}{\sum_{t= \teta+1}^{T} \epsilon_{\ell,t}} \,.
\end{align*} 
Since $\BDl(p_{\ell}^*, p_{\ell,\teta+1})$ and $\teta$ are finite, the condition $\lim_{T \to \infty}\sum_{t=1}^{T} \epsilon_{\ell,t} = \infty $ implies that $\lim_{T \to \infty}\sum_{t=\teta+1}^{T} \epsilon_{\ell,t} = \infty$, and the condition $\lim_{T \to \infty}\sum_{t=1}^{T} \epsilon_{\ell,t}^{2} < \infty $ implies that $\lim_{T \to \infty}\sum_{t=\teta+1}^{T} \epsilon_{\ell,t}^{2} <\infty$. Hence,
 $\frac{\sum_{t= \teta+1}^{T} \epsilon_{\ell,t}^{2}}{\sum_{t= \teta+1}^{T} \epsilon_{\ell,t}} = 0$ as $T\to \infty$. Finally, because $\ceta >0$, as $T\to \infty$, the above left hand side goes to zero and the  right hand side goes to $-\ceta < 0$. This is a contradiction, implying that our original assumption $|\Delta_{\ell}| > 0$ cannot hold, and hence $\Delta_{\ell} = \Delta_{-\ell} = 0$. 
 \Halmos
 
 
 
 \subsection{Proof of Theorem \ref{thm:OMD:rateDecStep}}
 \label{sec:technical:5.2}
Recall Equation (\ref{eq:OMD:gradDiffEq}): $ g_{i}^*- g_{i,t} 
    ~=~ 2\beta_{i} \left( p_{i}^{*} - p_{i,t}\right)-  \delta_{i}\left(p_{-i}^{*} -  p_{-i,t}\right) - \gamma_{i} \left(r^{*} - r_{t} \right)$.
Combining this with Corollary \ref{cor:SNEBregmanUpdate}, we obtain
\begin{align*}
   & \BDi(p_{i}^*, p_{i,t+1}) \\
     ~\leq~ & \BDi(p_{i}^*, p_{i,t}) -  \epsilon_{i,t} \left( 2\beta_{i}\left(p_{i}^* - p_{i,t} \right)^2 - 
    \delta_{i} \left(p_{-i}^{*} -  p_{-i,t}\right) \left(p_{i}^* - p_{i,t} \right)  - \gamma_{i} \left(r^{*} - r_{t} \right) \left(p_{i}^* - p_{i,t} \right)
    \right)  + \frac{\left(\epsilon_{i,t}g_{i,t}\right)^2}{2\sigma_{i}} \nonumber \\ 
    %   ~\leq~ &  \BDi(p_{i}^*, p_{i,t}) -  \epsilon_{i,t} \left( 2\beta_{i}\left(p_{i}^* - p_{i,t} \right)^2 - 
    % \frac{\delta_1}{2} \left(\left(p_{2}^{*} -  p_{2,t-1}\right)^2 +  \left(p_{i}^* - p_{i,t} \right)^2 \right) \right) \nonumber \\ 
    % ~~~~ & - \epsilon_{i,t} \gamma_{i} \left(r^{*} - r_{t} \right) \left(p_{i}^* - p_{i,t} \right)  + \frac{\left(\epsilon_{i,t}g_{i,t}\right)^2}{2\sigma_{i}} \nonumber \\ 
    ~\overset{(a)}{\leq}~ &  \BDi(p_{i}^*, p_{i,t}) -  \epsilon_{i,t} \left(\frac{4\beta_{i} - \delta_{i}}{2} \left(p_{i}^* - p_{i,t} \right)^2 - 
    \frac{\delta_{i}}{2} \left(p_{-i}^{*} -  p_{-i,t}\right)^2 \right) + \epsilon_{i,t} \gamma_{i} \left(r^{*} - r_{t} \right) \left(p_{i}^* - p_{i,t} \right)  + \frac{\left(\epsilon_{i,t}g_{i,t}\right)^2}{2\sigma_{i}} \,.
    % ~\overset{(a)}{\leq}~ &  \BDi(p_{i}^*, p_{i,t}) -  \frac{3n}{t} \left(p_{i}^* - p_{i,t} \right)^2 + \frac{n}{t} \left(p_{-i}^{*} -  p_{-i,t-1}\right)^2   + \frac{n}{t}\left(r^{*} - r_{t} \right)^2   + \frac{\left(\epsilon_{i,t}g_{i,t}\right)^2}{2\sigma_{i}} \\
    % ~\overset{(b)}{\leq}~ &  \BDi(p_{i}^*, p_{i,t}) -  \frac{3n}{t} \left(p_{i}^* - p_{i,t} \right)^2 + \frac{n}{t} \left(p_{-i}^{*} -  p_{-i,t-1}\right)^2   + \frac{n}{t}\left(r^{*} - r_{t} \right)^2 +  \left(\epsilon_{i,t}\right)^2 \V
\end{align*}

% \negin{Let's assume that we don't apply the bounds on $\epsilon_{i,t}$ yet. What we get is 
% \begin{align*}
%    \BDi(p_{i}^*, p_{i,t+1}) 
%      &~\leq~\BDi(p_{i}^*, p_{i,t}) -  \epsilon_{i,t} \left(\frac{4\beta_{i} - \delta_{i}}{2} \left(p_{i}^* - p_{i,t} \right)^2 - 
%     \frac{\delta_{i}}{2} \left(p_{-i}^{*} -  p_{-i,t}\right)^2 \right) \nonumber \\ 
%     ~~~~ & + \epsilon_{i,t} \gamma_{i} \left(r^{*} - r_{t} \right) \left(p_{i}^* - p_{i,t} \right)  + \frac{\left(\epsilon_{i,t}g_{i,t}\right)^2}{2\sigma_{i}}
% \end{align*}
% Summing across $i = 1,2$, we have and assuming $\epsilon_{1, t}= \epsilon_{2,t} =\epsilon_{t}$, we get
% \begin{align*}
%   |p^*-p_{t+1}|^2 
%      &~\leq~ |p^*-p_t|^2 -  \epsilon_t \left(\frac{4\beta_1-\delta_1-\delta_2}{2}\right)(p_1^*-p_{1,t})^2-\epsilon_t\left(\frac{4\beta_2-\delta_2-\delta_1}{2}\right)(p_2^*-p_{2,t})^\\
%      &+\epsilon_t \gamma_2(r^*-r_t)(p_2-p_{2,t}^*)+\epsilon_t \gamma_1(r^*-r_t)(p_1-p_{1,t}^*)+ \frac{\left(\epsilon_{t}g_{1,t}\right)^2}{2\sigma_{1}}+\frac{\left(\epsilon_{t}g_{2,t}\right)^2}{2\sigma_{2}}
% \end{align*}}


where in (a) we used the basic inequality $AB \leq (A^{2} + B^{2})/2$ for $A= p_{-i}^{*} -  p_{-i,t}$ and $B = p_{i}^* - p_{i,t}$.

Now, consider the step-size sequences $\{\epsilon_{i,t}\}_{t}$ that satisfy
\begin{align}
\label{eq:OMD:stepsizeRange}
    \frac{1}{t+1}\cdot \frac{10}{4\beta_{i} - \delta_{i} }~\leq~ \epsilon_{i,t} ~\leq~ \frac{1}{t+1}\cdot \frac{2}{\max\{\delta_{i},\gamma_{i}\}},\quad i = 1,2\,.
\end{align}
Equation (\ref{eq:OMD:stepsizeRange}) holds due to the fact that $\beta_{i} > \margin( \delta_{i} + \gamma_{i}) > 0$ and $\margin\geq 2$, which further implies $2\left( 4\beta_{i} - \delta_{i} \right) > 8\margin(\delta_{i} + \gamma_{i}) - 2\delta_{i}  > 10(\delta_{i} + \gamma_{i}) > 10\max\{\delta_{i},\gamma_{i}\}$. This leads to
\begin{align*}
    &\BDi(p_{i}^*, p_{i,t+1}) \\
    ~\leq~ &  \BDi(p_{i}^*, p_{i,t}) -  \frac{5}{t+1} \left(p_{i}^* - p_{i,t} \right)^2 + \frac{1}{t+1} \left(p_{-i}^{*} -  p_{-i,t}\right)^2  + \frac{2}{t+1} \left(r^{*} - r_{t} \right) \left(p_{i}^* - p_{i,t} \right)    + \frac{\left(\epsilon_{i,t}g_{i,t}\right)^2}{2\sigma_{i}} \\
    ~\overset{(a)}{\leq}~ &  \BDi(p_{i}^*, p_{i,t}) -  \frac{5}{t+1} \left(p_{i}^* - p_{i,t} \right)^2 + \frac{1}{t+1} \left(p_{-i}^{*} -  p_{-i,t}\right)^2   + \frac{2}{t+1} \left(r^{*} - r_{t} \right) \left(p_{i}^* - p_{i,t} \right)  +  \frac{\V}{2(t+1)^{2}}
    \,, 
\end{align*}
where in (a) we take some $\V > \max_{i\in\{1,2\},t\in \N^{+}}\frac{4g_{i,t}^{2}}{\sigma_{i}\max\{\delta_{i},\gamma_{i}\}^{2}}$  %\negin{$\max\{\delta_{i},\gamma_{i}\}$
%should be bounded away from zero.}
for all $i,t$ by using the fact that $p_{i,t},r_{t} \in \mathcal{P}$. Summing across $i = 1,2$, we have
\begin{align*}
     \sum_{i=1,2}\BDi(p_{i}^*, p_{i,t+1}) 
    ~\leq~ &   \sum_{i=1,2}\BDi(p_{i}^*, p_{i,t}) -  \frac{4}{t+1} \norm{\bm{p}^{*} - \bm{p}_{t}}^{2}  + \frac{2}{t+1} \left(r^{*} - r_{t} \right) \left(p_{1}^{*} - p_{1,t}+ p_{2}^{*} - p_{2,t} \right)  +  \frac{\V}{(t+1)^{2}}\\
    %  ~\leq~ &   \sum_{i=1,2}\BDi(p_{i}^*, p_{i,t}) -  \frac{4}{t+1} \norm{\bm{p}^{*} - \bm{p}_{t}}^{2}  + \frac{1}{t+1} \left(r^{*} - r_{t} \right)^{2} + \frac{1}{t} \left(p_{1}^{*} - p_{1,t}+ p_{2}^{*} - p_{2,t} \right)^{2} +  \frac{\V}{(t+1)^{2}}\\
     ~\overset{(a)}{\leq}~ &   \sum_{i=1,2}\BDi(p_{i}^*, p_{i,t}) -  \frac{2}{t+1} \norm{\bm{p}^{*} - \bm{p}_{t}}^{2}  + \frac{1}{t+1} \left(r^{*} - r_{t} \right)^{2} +  \frac{\V}{(t+1)^{2}}
    \,, 
\end{align*}
where in inequality (a) we applied  $C(A+B) \leq \frac{C^{2}}{2} + \frac{(A+B)^{2}}{2} \leq \frac{C^{2}}{2} + A^{2} + B^{2}$ for $A = p_{1}^{*} - p_{1,t}$, $B = p_{2}^{*} - p_{2,t}$ and $C =r^{*} - r_{t} $.


When $R_{i}(z) = z^{2}$, we have $\BDi(p,p') = (p-p')^{2}$. Therefore, denoting $x_{t} =   \sum_{i=1,2}\BDi(p_{i}^{*}, p_{i,t}) = \norm{\bm{p}^{*} - \bm{p}_{t}}^{2}$ and $x_{n,t} = \left(r^{*} - r_{t} \right)^{2}$, the equation above yields
\begin{align}
\label{eq:OMD:rateIteration0}
     x_{t+1} ~\leq~  \left(1-\frac{2}{t+1}\right)x_{t} +\frac{1}{t+1}x_{n,t} + \frac{\V}{(t+1)^{2}}\,.
\end{align}

We will show via induction that $x_{t}\leq \frac{\const}{t}$ for some $\const > 0$ and any $t\in \N^{+}$. The proof is constructive and will rely on the following definitions, whose motivations will later be clear.  



Fix  $\NN = \left \lceil\frac{a}{1-a}\right \rceil + 1$, $\MN = \left\lceil \frac{\frac{a}{1-a}(\NN+1)}{\NN - \frac{a}{1-a}}\right\rceil$,  and take any $\ourrho$ so that $\max\left\{\theta_{1}, \theta_{2}\right\} < \ourrho < 1$. Here,  $\lceil x \rceil = \min \{y \in \N^{+}: y \geq x \}$ for any $x \in \R$. Note that $\NN$ is bounded as $a$ is bounded away from 1.
%\negin{How does $\const$ scale with $a$ and $\max\{\theta_1, \theta_2\}$? Does it go to infinity as $a$ goes to one?}
Define
\begin{align}
    & \trho \defeq \min\left\{\tau \in \N^{+}: \tau \geq \NN \text{ and } \frac{(\NN+1)\log(\tau-\NN-1)}{\tau} \leq  \frac{\ourrho}{\max\{\theta_{1}, \theta_{2} \}}-1 \right\} \label{def:OMD:Trho}\\
    & \Q \defeq (1-a)\max\{\theta_{1}, \theta_{2}\}\sum_{\tau=1}^{\NN+\MN-1} \frac{a^{-\tau}}{\tau}\,. \label{eq:OMD:Q}
\end{align}
%\negin{Feel free to change the notation for $\Q$ as I was not sure what the nest notation is here. I chose $\NN$ for $N$ to remind the readers (1) $N$ depends on $a$ and (2) we are talking about a ration. I made several notation changes here. Please review carefully to make sure I did not miss anything.  } \jasoncom{I changed this to $u$ because $p$ and $q$ look very similar.}
Note that $\trho$ is bounded because $\max\{\theta_1, \theta_2\}$ is bounded away from one. Further, since $\NN$ and $\ourrho$ are constant, and $\log(t) =o(t)$, it is easy to see that $\trho$ exists. Furthermore, define $\const \defeq\frac{ 2 \tildet (\Bar{p} -\underline{p})^{2} + \V + 1}{1-\ourrho}$ and
\begin{align*}
    & \tildet \defeq \min \Bigg\{\tau >  \max\left\{\NN + \MN, \trho\right\}: \left. (t-\NN) \cdot \left(2(\Bar{p} -\underline{p})^{2} + \Q\cdot \frac{ 2t \cdot (\Bar{p} -\underline{p})^{2} + \V + 1}{1-\ourrho}\right) < a^{-t}\quad, \text{for } \forall t \geq \tau \right\}\,.
    % &  \const \defeq\frac{ 2 \tildet (\Bar{p} -\underline{p})^{2} + \V + 1}{1-\ourrho}\,.
\end{align*}
 Such $\tildet$ must exist because  the left hand side is quadratic in $t$, while the right hand side is exponential in $t$ for $a \in (0,1)$. We provide an illustration for the size of $\const$ w.r.t. memory parameter $a$ and $\max\{\theta_{1},\theta_{2}\}$ in Figure \ref{fig:rate_constant} of Appendix \ref{app:sec:addFigures}. These definitions of $\tildet$ and $\const$ imply the following:
\begin{align}
   & a^{t}\left(2(\Bar{p} -\underline{p})^{2} + \Q\const\right) < \frac{1}{t-\NN} \quad \forall t \geq \tildet \label{eq:OMD:tildeT1}\\
   &   2 \tildet (\Bar{p} -\underline{p})^{2} + \V + 1 + \ourrho \const = \const \label{eq:OMD:tildeT2}\\
   &  \const > 2\tildet (\Bar{p} -\underline{p})^{2} \label{eq:OMD:tildeT3}
   \,.
\end{align}
Here, Equation (\ref{eq:OMD:tildeT1}) is due to the following: plugging the definition of $\const$ into that of $\tildet$ we get
$(\tildet-\NN) \cdot \left(2(\Bar{p} -\underline{p})^{2} + \Q\const \right) < a^{-\tildet}$, and since $\const = \frac{ 2 \tildet (\Bar{p} -\underline{p})^{2} + \V + 1}{1-\ourrho} \leq   \frac{ 2t \cdot (\Bar{p} -\underline{p})^{2} + \V + 1}{1-\ourrho}$ for any $t \geq \tildet > \NN$, we have  
$$(t-\NN)\left(2(\Bar{p} -\underline{p})^{2} + \Q\const\right) \leq  (t-\NN)\left(2(\Bar{p} -\underline{p})^{2} + \Q\cdot \frac{ 2t \cdot (\Bar{p} -\underline{p})^{2} + \V + 1}{1-\ourrho}\right) \overset{(a)}{<} a^{-t}\,,$$
where (a) follows from the definition of $\tildet$. Equation (\ref{eq:OMD:tildeT2}) directly follows from the definition of $\const$. Equation (\ref{eq:OMD:tildeT3}) follows because $\ourrho \in (0,1)$ and hence $\const = \frac{ 2 \tildet (\Bar{p} -\underline{p})^{2} + \V + 1}{1-\ourrho} > 2 \tildet (\Bar{p} -\underline{p})^{2} + \V + 1 >  2 \tildet (\Bar{p} -\underline{p})^{2}$. Hence, this implies that  $x_{t} \leq 2(\Bar{p} -\underline{p})^{2}< \frac{\const}{t}$ for any $t = 1\dots \tildet$, where we recall $x_{t} = \norm{\bm{p}^{*} - \bm{p}_{t}}^{2}$.

Consider $t\ge \tildet$.  We will now show via induction that $x_{t+1} \leq \const/(t+1)$ using our induction hypothesis  that 
% $x_{t}\leq {\const}/{t}$ using the induction hypothesis
$x_{\tau}\leq \const/\tau$ holds for all $\tau =1, \dots, t$. % and our base case 
% is $x_{\tau}\leq \const/\tau$ for $\tau=1, 2, \ldots, \tildet$.
 %We will further show that  $x_{T+1} \leq \const/(T+1)$. 
Note that the base case $x_{t} \leq 2(\Bar{p} -\underline{p})^{2}< \frac{\const}{t}$ for any $t = 1\dots \tildet$ is trivially true as we just discussed. Then, multiplying $t(t+1)$ on both sides of the recurrence relation in Equation (\ref{eq:OMD:rateIteration0}) and telescoping from $\tildet$  to $t$, we have
\begin{align}
\label{eq:OMD:rateIteration}
     t(t+1)x_{t+1} ~\leq~&  (t-1)t x_{t} +t x_{n,t} + \V 
     ~\leq~  (t-2)(t-1) x_{t-1} + \sum_{\tau=t-1}^{t} t x_{n,\tau} + 2\V \nonumber \\
    %   ~\vdots~& \nonumber \\
     ~\overset{(a)}{\leq}~& (\tildet-1) \tildet\cdot x_{\tildet} + \sum_{\tau=\tildet}^{t} \tau x_{n,\tau} + (t - \tildet+1)\V  
     ~\leq~ (\tildet-1) \tildet \cdot x_{\tildet} + \sum_{\tau= \tildet}^{t} \tau x_{n,\tau} + t\V  \,.
\end{align}
Here, (a) follows from telescoping. We will now bound $x_{n,\tau}$ for all $\tau = \tildet\dots t$. Using the definition $r^{*} = \theta_{1}p_{1}^{*} + \theta_{2}p_{2}^{*}$, we get
\begin{align*}
    r^{*} - r_{\tau+1} ~=~   r^{*} - ar_{\tau}-(1-a)\left(\theta_{1}p_{1,\tau} + \theta_{2}p_{2,\tau} \right) 
     ~=~   a\left( r^{*} - r_{\tau}\right) -(1-a)\left(\theta_{1}\left(p_{1}^{*} - p_{1,\tau}\right) + \theta_{2}\left(p_{2}^{*} - p_{2,\tau}\right)\right)
      \,.
\end{align*}
By convexity, we further have for any $\tau = 1\dots t$,
\begin{align*}
x_{n,\tau+1} = \left(r^{*} - r_{\tau+1}\right)^{2}  ~\leq~ &  a x_{n,\tau} + (1-a)\left(\theta_{1}\left(p_{1}^{*} - p_{1,\tau}\right) + \theta_{2}\left(p_{2}^{*} - p_{2,\tau}\right)\right)^{2}\\
 ~\leq~ & a x_{n,\tau} + (1-a)\left(\theta_{1}\left(p_{1}^{*} - p_{1,\tau}\right)^{2} + \theta_{2}\left(p_{2}^{*} - p_{2,\tau}\right)^{2}\right)\\
 ~\leq~ & a x_{n,\tau} + (1-a)\max\{\theta_{1}, \theta_{2}\}x_{\tau}
 ~\overset{(a)}{\leq}~ a x_{n,\tau} + (1-a)\max\{\theta_{1}, \theta_{2}\}\frac{\const}{\tau}\,,
\end{align*}
where (a) follows from the induction hypothesis, i.e., $x_{\tau}\leq \const/\tau$ holds for all $\tau =1 \dots t$. Using a telescoping argument, we then have for any $t \geq \tildet$,
\begin{align*}
    x_{n, t+1}~\leq~ &a x_{n,t} + (1-a)\max\{\theta_{1}, \theta_{2}\}\frac{\const}{t} 
    % ~\leq~ & a^2x_{n, t-1}+ a(1-a)\const\max\{\theta_1, \theta_2\}\left(\frac{1}{t} + \frac{a}{t-1}\right)\\
    % ~\leq~ & a^2x_{n, t-1}+ (1-a)\const\max\{\theta_1, \theta_2\}\sum_{\tau=t-1}^{t}\frac{a^{t-\tau}}{\tau}
    % & \vdots \\
     ~\leq~ a^{t}x_{n,1} +(1-a) \const\max\{\theta_{1}, \theta_{2}\} \sum_{\tau=1}^{t} \frac{a^{t-\tau}}{\tau}\\
     ~=~ & a^{t}x_{n,1}  +(1-a)a^{t} \const\max\{\theta_{1}, \theta_{2}\}\left( \sum_{\tau=1}^{\NN+\MN-1} \frac{a^{-\tau}}{\tau} + \sum_{\tau=\NN+\MN}^{t} \frac{a^{-\tau}}{\tau} \right)\\
      ~\overset{(a)}{=}~ & a^{t}\left( x_{n,1} + \Q \const\right) +  (1-a)a^{t} \const\max\{\theta_{1}, \theta_{2}\}
      \sum_{\tau=\NN+\MN}^{t} \frac{a^{-\tau}}{\tau}\\\
       ~\leq~ & a^{t}\left(2(\Bar{p}-\underline{p})^{2}+ \Q \const\right) +  (1-a)a^{t} \const\max\{\theta_{1}, \theta_{2}\}
      \sum_{\tau=\NN+\MN}^{t} \frac{a^{-\tau}}{\tau}\\
       ~\overset{(b)}{\leq}~ & \frac{1}{t-\NN} +  (1-a)a^{t} \const\max\{\theta_{1}, \theta_{2}\}
      \sum_{\tau=\NN+\MN}^{t} \frac{a^{-\tau}}{\tau}
     ~\overset{(c)}{\leq}~  \frac{1 + \max\{\theta_{1}, \theta_{2}\} \const}{t-\NN}\,.
\end{align*}
Here, (a) follows from the definition of $\Q$ in Equation (\ref{eq:OMD:Q}); (b) follows from Equation (\ref{eq:OMD:tildeT1}); and (c) evokes Lemma \ref{lem:boundSum} since $t \geq \tildet \geq \NN + \MN$.
Applying this upper bound on $x_{n,t}$ in Equation (\ref{eq:OMD:rateIteration}) we have
\begin{align*}
      t(t+1)x_{t+1} 
     ~\leq~& (\tildet-1) \tildet \cdot x_{\tildet} + \left(1 + \max\{\theta_{1}, \theta_{2}\} \const\right) \sum_{\tau=\tildet}^{t} \frac{\tau}{\tau-\NN-1} + t\V \nonumber \\
     ~=~& (\tildet-1) \tildet\cdot x_{\tildet} + \left(1 + \max\{\theta_{1}, \theta_{2}\} \const\right) \sum_{\tau = \tildet}^{t} \left(1 + \frac{\NN+1}{\tau-\NN-1}\right) + t\V \nonumber\\
     ~\overset{(a)}{\leq}~& (\tildet-1) \tildet\cdot x_{\tildet} + \left(1 + \max\{\theta_{1}, \theta_{2}\} \const\right) \left(t + (\NN+1)\log(t-\NN-1)\right) +t\V
     \,.
\end{align*}
 where (a) follows from $\sum_{\tau = \tildet}^{t}\frac{1}{\tau-\NN-1} \leq \int_{\tildet-1}^{t}\frac{1}{\tau-\NN-1}  d\tau \leq \log(t-\NN-1) $ since $\tildet\geq \NN+3$. Dividing both sides of the above equation by $t(t+1)$, and using the fact that $x_{t}\leq 2(\Bar{p} -\underline{p})^{2}$ for any $t$, we have
 \begin{align*}
     x_{t+1}
     ~\leq ~ & \left(\frac{2(\tildet-1) \tildet(\Bar{p} -\underline{p})^{2}}{t} + \V \right)\cdot \frac{1}{t+1} + \frac{1 + \max\{\theta_{1}, \theta_{2}\} \const\left(1  + \frac{(\NN+1)\log(t-\NN-1)}{t}\right)}{t+1}\\
      ~\overset{(a)}{\leq}~ &  \frac{2\tildet (\Bar{p} -\underline{p})^{2} + \V + 1 + \max\{\theta_{1}, \theta_{2}\} \const\left(1  + \frac{(\NN+1)\log(t-\NN-1)}{t}\right)}{t+1}\\
       ~\overset{(b)}{\leq}~ &  \frac{2\tildet (\Bar{p} -\underline{p})^{2} + \V + 1 + \ourrho \const}{t+1}
        ~\overset{(c)}{=}~   \frac{\const}{t+1}
      \,.
 \end{align*}
Here, (a) follows from the fact that $t\geq \tildet$, so $\frac{2(\tildet-1) \tildet(\Bar{p} -\underline{p})^{2}}{t} + \V\leq 2\tildet (\Bar{p} -\underline{p})^{2} + \V$; (b) follows from $t\geq \tildet\geq \trho$ so that $\frac{(\NN+1)\log(t-\NN-1)}{t} \leq  \frac{\ourrho}{\max\{\theta_{1}, \theta_{2}\}}-1$ according to Equation (\ref{def:OMD:Trho}); finally, (c) follows from Equation (\ref{eq:OMD:tildeT2}).
\Halmos


==> 09_tatonnement.tex <==
\subsection{Firms acting myopically under incomplete information}
\begin{theorem}
\label{thm:tatonnementconvergence}
Assume both firms are myopic under incomplete information and follow a Tatonnement update scheme to set prices $\bm{p}^{t,\text{TU}} = (p_1^{t,\text{TU}}, p_2^{t,\text{TU}})$ under reference price $r^t$ in period $t$, where for $i = 1,2$
$$p_i^{t,\text{TU}} = \psi_i\left(p_{-i}^{t-1,\text{TU}},r^{t}\right)\,.$$ Then the reference price converges to some steady state $r^{\infty,\text{TU}}$ regardless of what the price priors 
$p_1^{0,\text{TU}}, p_2^{0,\text{TU}}$ are for both firms. Moreover, 
$$ r^{\infty,\text{TU}} = r^{\infty,\text{NE}} \in [0,R]\,,$$
where $r^{\infty,\text{NE}}$ is defined in Theorem \ref{thm:NEconvergence}.
\end{theorem}
\begin{proof}[Proof of Theorem \ref{thm:tatonnementconvergence}]
For simplicity, we omit the superscript ``TU'' since the context is clear that we are considering the tatonnement update scheme. According the the best response functions shown in Equation (\ref{eq:bestresponse}), we have
\begin{align}
\label{eq:bestresponseTU}
 p_1^{t+1} = \psi_1(p_2^{t},r^{t+1}) = \frac{\alpha_1 + \delta_1 p_2^{t} + \gamma_1 r^{t+1} }{2\beta_1} ~~~~,~~~~
p_2^{t+1} =\psi_2(p_1^{t},r^{t+1}) = \frac{\alpha_2 + \delta_2 p_1^{t} + \gamma_2 r^{t+1} }{2\beta_2} \,,
\end{align}
where $r^{t+1} = ar^{t} + (1-a)\left(\theta_1 p_1^{t} + \theta_2 p_2^{t}\right)$. Substituting this into Equation (\ref{eq:bestresponseTU}) and writing the equalities as a linear system, we have
\begin{align}
\underbrace{
\begin{pmatrix}
p_1^{t+1}\\[0.7em]
p_2^{t+1} \\[0.7em]
r^{t+1}
\end{pmatrix}}_{\mathbf{X}_{t+1}} = \underbrace{\begin{pmatrix}
\frac{(1-a)\theta_1 \gamma_1}{2\beta_1}  & \frac{\delta_1 +(1-a)\theta_2 \gamma_1}{2\beta_1} &\frac{a \gamma_1}{2\beta_1} \\[0.7em]
\frac{\delta_2 + (1-a)\theta_1 \gamma_2}{2\beta_2}  & \frac{(1-a)\theta_2 \gamma_2}{2\beta_2} &\frac{a \gamma_2}{2\beta_2}\\[0.7em]
(1-a)\theta_1 & (1-a)\theta_2 & a
\end{pmatrix}}_{\mathbf{A}} \underbrace{\begin{pmatrix}
p_1^{t} \\[0.7em]
p_2^{t} \\[0.7em]
r^{t}
\end{pmatrix}}_{\mathbf{X}_{t}} + \underbrace{\begin{pmatrix}
\frac{\alpha_1}{2\beta_1}\\[0.7em]
\frac{\alpha_2}{2\beta_2} \\[0.7em]
0
\end{pmatrix}}_{\mathbf{C}}\,.
\end{align}
We first consider the characteristic function of the matrix $\mathbf{A}$, namely $|\mathbf{A} - \lambda \mathbf{I}|$ where $\mathbf{I}$ is the identity matrix.
\begin{align}
\label{eq:TUlinsystem}
   & \left|\mathbf{A} - \lambda \mathbf{I}\right| \nonumber\\
~=~ & \left(\frac{(1-a)\theta_1 \gamma_1}{2\beta_1} - \lambda \right) \cdot \left|\begin{pmatrix}
\frac{(1-a)\theta_2 \gamma_2}{2\beta_2} - \lambda &\frac{a \gamma_2}{2\beta_2}\\[0.7em]
(1-a)\theta_2 & a - \lambda
\end{pmatrix} \right| \nonumber \\
& ~~~~ -
\frac{\delta_1 +(1-a)\theta_2 \gamma_1}{2\beta_1}  \cdot \left| \begin{pmatrix}
\frac{\delta_2 + (1-a)\theta_1 \gamma_2}{2\beta_2} &\frac{a \gamma_2}{2\beta_2}\\[0.7em]
(1-a)\theta_1 &  a - \lambda 
\end{pmatrix}\right| + \frac{a\gamma_1}{2\beta_1} \left|\begin{pmatrix}
\frac{\delta_2 + (1-a)\theta_1 \gamma_2}{2\beta_2}  & \frac{(1-a)\theta_2 \gamma_2}{2\beta_2} - \lambda\\[0.7em]
(1-a)\theta_1 & (1-a)\theta_2 
\end{pmatrix}\right| \nonumber \\
~=~& -\lambda^3 + \left(\frac{(1-a)\theta_1\gamma_1}{2\beta_1}+\frac{(1-a)\theta_2\gamma_2}{2\beta_2} + a\right)\lambda^2 + \frac{(1-a)\left(\theta_1\delta_1\gamma_2 + \theta_2\delta_2\gamma_1 \right)}{4\beta_1 \beta_2} \lambda + \frac{(1-a)\delta_1\delta_2}{4\beta_1\beta_2} \,.
\end{align}
Now, considering $\lambda = 1$, we have
\begin{align}
\label{eq:A-Iinvertible}
    \left|\mathbf{A} - \mathbf{I}\right| ~=~ & (1-a)\left(-1 +  \frac{\theta_1\gamma_1}{2\beta_1}+\frac{\theta_2\gamma_2}{2\beta_2}  + \frac{\theta_1\delta_1\gamma_2 + \theta_2\delta_2\gamma_1 }{4\beta_1 \beta_2}+ \frac{\delta_1\delta_2}{4\beta_1\beta_2} \right)\nonumber\\
     ~=~ & -(1-a)\cdot\frac{\left(2\beta_1 - \theta_1 \gamma_1\right)\left(2\beta_2 - \theta_2 \gamma_2\right) - \left(\theta_2\gamma_1 +\delta_1\right)\left(\theta_1\gamma_2 +\delta_2\right)}{4\beta_1\beta_2}\,.
\end{align}
According to Equation \ref{def:RAdemand}, we have $\beta_i > \delta_i +  \gamma_i $ for $i = 1,2$ so
$$ \left(2\beta_1 - \theta_1 \gamma_1\right) - \left(\theta_2\gamma_1 +\delta_1\right) = 2\beta_1  - \delta_1 -  \gamma_1 > \beta_1 >0\,.$$
Similarly, $ \left(2\beta_2 - \theta_2 \gamma_2\right) - \left(\theta_1\gamma_2 +\delta_2\right) > 0$. Therefore, since $a\in(0,1)$, Equation (\ref{eq:A-Iinvertible}) implies $ \left|\mathbf{A} - \mathbf{I}\right| < 0$, which means the matrix $\mathbf{A} - \mathbf{I}$ is invertible. Hence, by rearranging terms in Equation (\ref{eq:TUlinsystem}) we have
\begin{align*}
  \mathbf{X}_{t+1} + \left(\mathbf{A} - \mathbf{I}\right)^{-1}\mathbf{C}= \mathbf{A}\left(\mathbf{X}_{t} + \left(\mathbf{A} - \mathbf{I}\right)^{-1}\mathbf{C} \right)\,,
\end{align*}
which further implies for $t \in \N^+$
\begin{align*}
    \mathbf{X}_{t} + \left(\mathbf{A} - \mathbf{I}\right)^{-1}\mathbf{C} = \mathbf{A}^{t-1}\left(\bm{X}_{1} + \left(\mathbf{A} - \mathbf{I}\right)^{-1}\mathbf{C} \right)\,,
\end{align*}
where $\mathbf{A}^{t-1}$ is the product of $t-1$ identical $\mathbf{A}$ matrices. According to Lemma \ref{lem:convergingA}, we have $\lim_{t\rightarrow \infty} \mathbf{A}^{t} = \mathbf{0}$. Therefore this implies 
\begin{align}
\label{eq:Xconvergence}
    \lim_{t\rightarrow \infty}\mathbf{X}_{t} = -  \left(\mathbf{A} - \mathbf{I}\right)^{-1}\mathbf{C}\,.
\end{align}{}
A direct calculation yields
\begin{align}
\label{eq:invertA-I}
    \left(\mathbf{A} - \mathbf{I}\right)^{-1} = \frac{1}{\left|\mathbf{A} - \mathbf{I}\right|} \begin{pmatrix}(1-a)\left(1 - \frac{\theta_2 \gamma_2}{2\beta_2} \right)
 & (1-a)\frac{\theta_2 \gamma_1 + \delta_1}{2\beta_1} &\frac{a \gamma_2 \delta_1}{4\beta_1 \beta_2}  + \frac{a \gamma_1}{2\beta_1}\\[0.7em]
(1-a)\frac{\theta_1 \gamma_2+\delta_2}{2\beta_2} & (1-a)\left(1 - \frac{\theta_1 \gamma_1}{2\beta_1} \right) &\frac{a \gamma_1\delta_2}{4\beta_1 \beta_2}  + \frac{a \gamma_2}{2\beta_2}\\[0.7em]
(1-a)\left(\frac{\delta_2 \theta_2}{2\beta_2} +\theta_1\right) & (1-a)\left(\frac{\delta_1 \theta_1}{2\beta_1} +\theta_2\right) & Z
\end{pmatrix}\,,
\end{align}
where $Z =1 - \frac{(1-a)\gamma_1\left(\theta_1 + \theta_2\delta_2 \right)}{2\beta_1}+\frac{(1-a)\gamma_2\left(\theta_2 + \theta_1\delta_1\right)}{2\beta_2} - \frac{\delta_1\delta_2}{4\beta_1\beta_2} $. Therefore, by Equations (\ref{eq:A-Iinvertible}),  (\ref{eq:Xconvergence}) and (\ref{eq:invertA-I}), we have 
\begin{align*}
       & \begin{pmatrix}
        p_1^{\infty}\\[0.7em]
        p_2^{\infty}\\[0.7em]
        r^{\infty}
        \end{pmatrix} \defeq \lim_{t\rightarrow \infty}\mathbf{X}_t  =  -  \left(\mathbf{A} - \mathbf{I}\right)^{-1}\mathbf{C}\\
        ~=~ & \frac{1}{\left(2\beta_1 - \theta_1 \gamma_1\right)\left(2\beta_2 - \theta_2 \gamma_2\right) - \left(\theta_2\gamma_1 +\delta_1\right)\left(\theta_1\gamma_2 +\delta_2\right)}
    \begin{pmatrix}
    2\alpha_1 \beta_2 - \alpha_1\theta_2 \gamma_2 + \alpha_2\left(\delta_1 +\theta_2\gamma_1\right)\\[0.7em]
     2\alpha_2 \beta_1  - \alpha_2 \theta_1\gamma_1 + \alpha_1\left(\delta_2 +\theta_1\gamma_2\right)\\[0.7em]
     \theta_1\left(2\alpha_1\beta_2 + \alpha_2\delta_1\right)+\theta_2\left(2\alpha_2\beta_1 + \alpha_1\delta_2\right)
\end{pmatrix}\,.
\end{align*}

 
\end{proof}


\begin{lemma}
\label{lem:convergingA}
$\lim_{t\rightarrow \infty} \mathbf{A}^{t} = \mathbf{0}$, where $\mathbf{A} \in R^{3\times 3}$ is defined in Equation (\ref{eq:TUlinsystem}).
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lem:convergingA}]
We let $\lambda_1,\lambda_2,\lambda_3$ be the eigenvalues of $\mathbf{A}$. Note that $\lambda_1,\lambda_2,\lambda_3$ may be real or complex. Nevertheless, the complex conjugate of a root (i.e. eigenvalue of $\mathbf{A}$) for the characteristic function $|\mathbf{A} -\lambda\mathbf{I}|$ is also a root/ eigenvalue, so we know that one of the eigenvalues must be real. Without loss of generality we assume $\lambda_1 \in \R$, while $\lambda_2,\lambda_3$ are complex conjugates, that is, $\lambda_2 = x + y\text{i}$  and $\lambda_3= x - y\text{i}$ for some $x,y\in\R$. 

Furthermore, we define the spectral radius $\rho(\mathbf{A})$ of $\mathbf{A}$ as $\rho(\mathbf{A}) = \max_{i=1,2,3}\{|\lambda_i|\}$,  where we recall for any complex number $z\in \mathbb{C}$, $|z|$ denotes its modulus. By the characteristic function in Equation (\ref{eq:TUlinsystem}) and using the fact that $|z_1\cdot z_2| =|z_1|\cdot|z_2| $for any two complex numbers $z_1,z_2\in \mathbb{C}$, we have
\begin{align}
   & (x^2 + y^2)\lambda_1 = \prod_{i=1}^3\lambda_i=  \frac{(1-a)\delta_1\delta_2}{4\beta_1\beta_2} \in \left(0, \frac{1-a}{4} \right) \subset\left(0,\frac{1}{4}\right)\,, \label{eq:spectralradius1}\\
   &(x^2 + y^2) + 2x\lambda_1 = \sum_{\substack{i,j = 1,2,3\\i\neq j}}\lambda_i\lambda_j = -
   \frac{(1-a)\left(\theta_1\delta_1\gamma_2 + \theta_2\delta_2\gamma_1 \right)}{4\beta_1 \beta_2} \in \left(-\frac{1-a}{2},0\right)\subset \left(-\frac{1}{2},0\right)\,, \label{eq:spectralradius2} \\
   & 2x + \lambda_1 = \sum_{i=1}^3\lambda_i= 
\frac{(1-a)\theta_1\gamma_1}{2\beta_1}+\frac{(1-a)\theta_2\gamma_2}{2\beta_2} + a \in (0,1) \label{eq:spectralradius3}\,,
\end{align}
where we used the fact that for $i=1,2$, $a,\theta_i, \delta_i, \gamma_i \in (0,1)$, $\beta_i > \delta_i + \gamma_i$ which implies $\frac{\delta_i}{\beta_i}, \frac{\gamma_i}{\beta_i} \in(0,1)$, and hence $0 < \frac{(1-a)\theta_1\gamma_1}{2\beta_1}+\frac{(1-a)\theta_2\gamma_2}{2\beta_2} + a < \frac{1-a}{2} + \frac{1-a}{2} + a = 1$. 


We will now show $x\in \left(-\frac{1}{2},0\right)$, $y^2 < \frac{1}{2}$, and $\lambda_1 \in \left(0,\frac{1}{3}\right)$. From Equations (\ref{eq:spectralradius1}) and (\ref{eq:spectralradius2}) we see that $\lambda_1 > 0$ and $x< 0$. We consider the following:
\begin{itemize}
    \item If $x \leq -\frac{1}{2}$, then by Equation (\ref{eq:spectralradius1}) we know that $0< \lambda_1 < 1$. But according to Equation (\ref{eq:spectralradius3}), this implies $2x + \lambda_1 < 0$, contradiction. hence $x\in \left(-\frac{1}{2},0\right)$.
    
    \item If $y^2 \geq \frac{1}{2}$, then by Equation (\ref{eq:spectralradius1}) we know that $0< \lambda_1 < \frac{1}{2}$. On the other hand, since we showed $x\in \left(-\frac{1}{2},0\right)$, we have $2x\lambda_1 \in \left(-\frac{1}{2},0\right)$. However, this implies $(x^2 + y^2) + 2x\lambda_1 > y^2 +  2x\lambda_1 > 0$, contradicting Equation (\ref{eq:spectralradius2}). Therefore $y^2 < \frac{1}{2}$.
    
    \item Finally, from Equation (\ref{eq:spectralradius1}), using the fact that $x\in \left(-\frac{1}{2},0\right)$ and $y^2 < \frac{1}{2}$ we can conclude $\lambda_1 < \frac{1}{3}$.
\end{itemize}
Hence, we can conclude that $|\lambda_2 | = |\lambda_3|= \sqrt{x^2 + y^2} < 1$ and $|\lambda_1| < 1$, which further implies the spectral radius $\rho(\mathbf{A}) < 1$. By Equation (7.10.5) of \cite{meyer2000matrix} we conclude $\lim_{t\rightarrow \infty} \mathbf{A}^{t} = \mathbf{0}$. 
\end{proof}


\subsection{Pricing for a strategic firm with complete information against myopic opponent with  incomplete information}
\begin{theorem}
\label{thm:bellmanconverge}
Assume, without loss of generality, firm 1  has complete information of the parameter set $\Omega = (\Omega_1, \Omega_2)$ defined in Equation (\ref{eq:infoset}), while firm 2 only knows its own set of parameters $\Omega_2$. Consider the setting where firm 2 myopically updates its prices through a tatonnement scheme, i.e. for $t\in \N^+$,
$$p_2^{t} = \psi_2\left(p_{1}^{t-1},r^{t}\right)\,,$$while firm 1 maximizes its long term profit via the optimization problem (or Sequence problem (SP))
 \begin{eqnarray*}
 (SP) & \sup_{\{p_1^{t}\}_t}  & \sum_{t = 1}^{\infty} \eta^{t}\pi_1\left(p_1^t, p_2^t, r^t\right) \\ 
     & \text{s.t.} & r^t = a r^{t-1} + (1-a)\left(\theta_1 p_1^{t-1} + \theta_2 p_2^{t-1} \right),~~~~ t\geq 2\\
     & & p_2^t = \psi_2\left(p_1^{t-1}, r^t\right),~~~~ t\geq 2\\
     & & p_2^1 = p_2, r^1 = r
\end{eqnarray*}
where $\eta \in (0,1)$ is a time discount factor. Then, the reference price $r^t$ will converge to some steady state $r^{\infty}$.
\end{theorem}
\begin{proof}[Proof of Theorem \ref{thm:bellmanconverge}]
Consider the Bellman Equation 
\begin{align}
\label{eq:bellman}
    V(p_2,r) = \max_{p}\left\{\pi_1\left(p,p_2,r\right) + \eta V\left(\psi_2\left(p, r\right),a r + (1-a)\left(\theta_1 p + \theta_2 p_2 \right)\right)\right\}\,.
\end{align}

 \begin{eqnarray*}
 V(p_2,r) = & \max_{p} & \left\{\pi_1\left(p,p_2,r\right) + \eta V\left(\Bar{p}_2, \Bar{p}\right)\right\} \\ 
     & \text{s.t.} &\Bar{p}_2 = \frac{\alpha_2 + \delta_2 p + \gamma_2 \Bar{p} }{2\beta_2} \\
     && \Bar{p} = a r + (1-a)\left(\theta_1 p + \theta_2 p_2 \right)\\
     & & \pi_1\left(p,p_2,r\right) = p\left(\alpha_1 - \beta_1 p + \delta_1 p_2 + \gamma_1 r \right)
\end{eqnarray*}

\end{proof}

==> scratch.tex <==
\begin{align}
    \label{eq:OMD:telescope}
   \frac{\sigma_{\ell}^2}{2}\left(|\Delta_{\ell}|- \eta \right)^2 ~\overset{(a)}{\leq}~& \BDi(p_{\ell}^*, p_{\ell,T+1}) \nonumber \\
    ~\leq~& \BDi(p_{\ell}^*, p_{\ell,T}) - \ceta \epsilon_{\ell,T} +  \V\epsilon_{\ell,T}^{2} \nonumber \\
    & \vdots \nonumber \\
   ~\leq~& \BDi(p_{\ell}^*, p_{\ell,\teta+1}) - \ceta\sum_{t= \teta+1}^{T} \epsilon_{\ell,t} +   \V\sum_{t= \teta+1}^{T} \epsilon_{\ell,t}^{2} \,,
\end{align}
where we take the absolute constant $\V > \max_{t \in \N,~ i=1,2} \frac{g_{\ell,t}^{2}}{2\sigma_{\ell}}$ which is possible as  the gradient $g_{\ell,t}$ is a linear function in all arguments and prices/ reference prices are bounded. Inequality 
(a) follows from strong convexity of $R_i$ so that
$$\BDi(p_{\ell}^*, p_{\ell,T+1}) \geq  \frac{\sigma_{\ell}^2}{2}\left(p_{\ell}^* - p_{\ell,T+1}\right)^{2} {\geq}   \frac{\sigma_{\ell}^{2}}{2}\left( \left| \Delta_{\ell}\right| - \eta\right)^{2}$$ where the second inequality 
follows because for any $t > \teta$, $|p_{\ell}^* - p_{\ell,t}| > |\Delta_{\ell} - \eta| \geq |\Delta_{\ell}| - \eta > 0$ by evoking the lower bound of $p_{\ell}^* - p_{\ell,t}$ in Equation (\ref{eq:OMD:priceLB}) and using the definition that $0 < \eta < \min_{\ell=1,2: \Delta_{\ell} \neq 0}\{ |\Delta_{\ell}|\}$. Rearranging terms in Equation \eqref{eq:OMD:telescope} and dividing both sides by $\sum_{t= \teta+1}^{T} \epsilon_{\ell,t}$ we get
the following for $i \in \{1,2\}$ s.t. $\Delta_{\ell} \neq 0$ \negin{Why are we repeating this ``s.t. $\Delta_{\ell} \neq 0$"?}:
\begin{align*}
   \frac{1}{\sum_{t= \teta+1}^{T} \epsilon_{\ell,t}} \left(\frac{\sigma_{\ell}^2}{2}\left(|\Delta_{\ell}|- \eta \right)^2 -\BDi(p_{\ell}^*, p_{\ell,\teta+1}) \right) ~\leq~   - \ceta +   \V \frac{\sum_{t= \teta+1}^{T} \epsilon_{\ell,t}^{2}}{\sum_{t= \teta+1}^{T} \epsilon_{\ell,t}} \,.
\end{align*} 
Since $\BDi(p_{\ell}^*, p_{\ell,\teta+1})$ and $\teta$ are finite, the condition $\lim_{T \to \infty}\sum_{t=1}^{T} \epsilon_{\ell,t} = \infty $ implies $\lim_{T \to \infty}\sum_{t=\teta+1}^{T} \epsilon_{\ell,t} = \infty$; on the other hand, the condition $\lim_{T \to \infty}\sum_{t=1}^{T} \epsilon_{\ell,t}^{2} < \infty $ implies $\lim_{T \to \infty}\sum_{t=\teta+1}^{T} \epsilon_{\ell,t}^{2} <\infty$. Hence,
 $\frac{\sum_{t= \teta+1}^{T} \epsilon_{\ell,t}^{2}}{\sum_{t= \teta+1}^{T} \epsilon_{\ell,t}} = 0$ as $T\to \infty$. Finally, because $\ceta >0$, as $T\to \infty$, the above left hand side goes to zero and the  right hand side goes to $-\ceta < 0$. This is a contradiction, implying that our original assumption of $\Delta_{\ell} \neq 0$ for some $i \in \{1,2\}$ cannot hold.
